Evaluating Feynman Integrals Using D-modules and Tropical Geometry

Feynman integrals play a central role in the modern scattering amplitudes research program. Advancing our methods for evaluating Feynman integrals will, therefore, strengthen our ability to compare theoretical predictions with data from particle accelerators such as the Large Hadron Collider. Motivated by this, the present manuscript purports to study mathematical concepts related to Feynman integrals. In particular, we present both numerical and analytical algorithms for the evaluation of Feynman integrals. The content is divided into three parts. Part I focuses on the method of DEQs for evaluating Feynman integrals. An otherwise daunting integral expression is thereby traded for the comparatively simpler task of solving a system of DEQs. We use this technique to evaluate a family of two-loop Feynman integrals of relevance for dark matter detection. Part II situates the study of DEQs for Feynman integrals within the framework of D-modules, a natural language for studying PDEs algebraically. Special emphasis is put on a particular D-module called the GKZ system, a set of higher-order PDEs that annihilate a generalized version of a Feynman integral. In the course of matching the generalized integral to a Feynman integral proper, we discover an algorithm for evaluating the latter in terms of logarithmic series. Part III develops a numerical integration algorithm. It combines Monte Carlo sampling with tropical geometry, a particular offspring of algebraic geometry that studies "piecewise-linear" polynomials. Feynman's i*epsilon-prescription is incorporated into the algorithm via contour deformation. We present an open-source program named Feyntrop that implements this algorithm, and use it to numerically evaluate Feynman integrals between 1-5 loops and 0-5 legs in physical regions of phase space.

==> dedication.tex <==
\begin{dedication}
To 
\end{dedication}


==> front-page.tex <==
\makeatletter
\begin{titlepage}
	\begin{center}
		\null
		\vfill
		
		{\Huge\bfseries\@displaytitle\par}
		
		\vspace{1.5cm}
		
		{\LARGE\itshape\@subtitle\par}
		
		\vspace{1.5cm}
		
		{\Large\href{\@authorURL}{\@author}\par}
		
		\vspace{1.5cm}
		
		{\large\itshape A dissertation submitted to}
		
		\vspace{1.5cm}
		
		{\large{\href{\@groupURL}{\@group}}\par}
		{\large{\href{\@schoolURL}{\@school}}\par}
		{\large{\href{\@universityURL}{\@university}}\par}
		
		\vspace{1.5cm}
				
		{\large January, 2023\par}
		
		\vfill
		\null
	\end{center}
\end{titlepage}
\makeatother

